Site-Specific MIMO Channel Generation via Diffusion and Flow Matching: Fidelity, Efficiency, and Downstream Utility

This paper explores the use of generative models to synthesize high-quality, site-specific multiple-input multiple-output (MIMO) channel data, addressing the high cost of the extensive measurement campaigns required to acquire real-world data for AI-native wireless networks. Two location-conditioned generative paradigms are compared: a conditional denoising diffusion implicit model (cDDIM), and a conditional flow matching model (cFMM). Both these models generate MIMO channel matrices conditioned on user coordinates, to preserve the spatial structure of the deployment site. The approaches are evaluated across three dimensions: statistical fidelity (including beam consistency and effective rank), generation efficiency, and utility in downstream tasks such as channel-state information compression and beam alignment. Results across diverse propagation scenarios (28 GHz and 3.5 GHz, both line-of-sight and non-line-of-sight) demonstrate that both models accurately capture site-specific characteristics, even when trained on scarce ground-truth data. Notably, cFMM achieves a quality comparable to cDDIM with roughly an order of magnitude less inference time. Augmenting scarce site-specific datasets with these synthetic channels yields hefty performance gains in downstream physical layer tasks compared to using scarce data alone or stochastic channels.

==> XX_notes_Paul.tex <==
\section*{\hl{Notes Paul}}

A structured view of the forward pass of the proposed architecture is provided in~\autoref{alg:unet}, which summarizes the interaction between the encoder–decoder backbone and the conditioning mechanisms. This unified architecture ensures that both generative models share identical representational capacity, enabling a fair comparison between stochastic diffusion and deterministic flow-based generation. 

\begin{algorithm}[t]
\caption{Forward pass of the conditional U-Net architecture}
\label{alg:unet}
\small
\begin{algorithmic}[1]
\REQUIRE Noisy/intermediate channel tensor $\mathbf{H}_t \in \mathbb{R}^{C \times H \times W}$, timestep $t$, coordinate condition $c_{\mathrm{xy}}$
\ENSURE Predicted tensor $\hat{\mathbf{H}}$

\STATE \textbf{// Encoder}
\STATE $x_0 \leftarrow \mathrm{ResBlock}(\mathbf{H}_t)$
\STATE $x_1 \leftarrow \mathrm{MaxPool}(\mathrm{ResBlock}(x_0))$
\STATE $x_2 \leftarrow \mathrm{MaxPool}(\mathrm{ResBlock}(x_1))$

\STATE \textbf{// Bottleneck representation}
\STATE $h \leftarrow \mathrm{GELU}(\mathrm{AvgPool}(x_2))$

\STATE \textbf{// Coordinate and time embeddings}
\STATE $e_c^{(1)} \leftarrow \phi_c^{(1)}(c_{\mathrm{xy}})$
\STATE $e_t^{(1)} \leftarrow \phi_t^{(1)}(t)$
\STATE $e_c^{(2)} \leftarrow \phi_c^{(2)}(c_{\mathrm{xy}})$
\STATE $e_t^{(2)} \leftarrow \phi_t^{(2)}(t)$

\STATE reshape embeddings to $\mathbb{R}^{C_k \times 1 \times 1}$ and broadcast spatially

\STATE \textbf{// Decoder stage 1}
\STATE $u_1 \leftarrow \mathrm{ConvTranspose}(h)$
\STATE $\tilde{u}_1 \leftarrow e_c^{(1)} \odot u_1 + e_t^{(1)}$
\STATE $u_2 \leftarrow \mathrm{ResBlock}(\mathrm{ResBlock}([\tilde{u}_1,\ x_2]))$

\STATE \textbf{// Decoder stage 2}
\STATE $\tilde{u}_2 \leftarrow e_c^{(2)} \odot u_2 + e_t^{(2)}$
\STATE $u_3 \leftarrow \mathrm{ResBlock}(\mathrm{ResBlock}([\tilde{u}_2,\ x_1]))$

\STATE \textbf{// Output projection}
\STATE $y \leftarrow \mathrm{ResBlock}([u_3,\ x_0])$
\STATE $\hat{\mathbf{H}} \leftarrow \mathrm{Conv}(y)$

\RETURN $\hat{\mathbf{H}}$
\end{algorithmic}
\end{algorithm}






%=========================================================

==> XX_notes_Sina.tex <==
\section*{\hl{Notes Sina}}

% =========================================================
\subsection*{Dataset Generation and Simulation Details}
% =========================================================

In this work, for the purpose of demonstrating the effectiveness of synthetic channel generation, ground-truth channel realizations are obtained from site-specific ray tracing based on a three-dimensional representation of a dense urban environment. The considered scene is extracted from a real cellular deployment and includes building geometries obtained from \gls{osm}~\cite{haklay2008openstreetmap}. For each \gls{ue} location, the ray tracer computes the propagation paths between the \gls{bs} and the \gls{ue}, including their delays, angles, and complex coefficients.

We consider three propagation scenarios: \emph{28\,GHz LoS}, \emph{3.5\,GHz LoS}, and \emph{3.5\,GHz LoS+NLoS}. All scenarios use the same urban scene, outdoor \gls{ue} sampling region, antenna dimensions, and ray-tracing mechanisms, but differ in carrier frequency and propagation condition. The \emph{LoS} setting includes only \gls{ue} locations with line-of-sight propagation, whereas the \emph{LoS+NLoS} setting includes both LoS and NLoS locations.

These scenarios are ordered by increasing modeling complexity. The 28\,GHz LoS case corresponds to a sparse mmWave propagation regime dominated by a small number of strong paths. The 3.5\,GHz LoS case introduces richer angular structure due to lower-frequency propagation, while the 3.5\,GHz LoS+NLoS case further introduces datapoints with stronger multipath.

The network and ray tracing configurations employed for generating the channel links between the \gls{bs} and the selected \glspl{ue} are summarized in Table~\ref{tab:network_rt_parameters}. In Sionna~RT, for user $u$, the frequency-domain channel response is computed from the complex path coefficients and delays as
\begin{equation}
H_u(f)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,e^{-j2\pi f \tau_{u,\ell}},
\label{eq:cfr_user}
\end{equation}
where $L_u$ is the number of valid propagation paths, $a_{u,\ell}\in\mathbb{C}$ is the complex coefficient of path $\ell$, $\tau_{u,\ell}$ is its propagation delay, and $f$ denotes the frequency variable.

\begin{table}[t]
\centering
\caption{Network and ray-tracing configuration parameters.}
\label{tab:network_rt_parameters}
\normalsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|p{0.48\columnwidth}|p{0.42\columnwidth}|}
\hline
\textbf{Parameter} & \textbf{Specification} \\
\hline
Frequencies & 3.5\,GHz and 28\,GHz \\
\hline
Maximum UE--BS distance & 100\,m \\
\hline
BS antenna elements (row, column) & $4 \times 8$ \\
\hline
UE antenna elements (row, column) & $2 \times 2$ \\
\hline
BS height & 25\,m\,(3.5\,GHz) 8.5\,m\,(28\,GHz) \\
\hline
UE height & 1.5\,m \\
\hline
Number of shooting rays & $5 \times 10^{6}$ \\
\hline
Maximum ray bounces & 3 \\
\hline
Ray types & LoS, specular reflection, diffraction \\
\hline
\end{tabular}
\end{table}


The dataset is generated from a single dense urban scene extracted from a real cellular deployment. The selected environment spans an area of $250 \times 250$ meters and contains detailed three-dimensional building geometries obtained from \gls{osm}~\cite{haklay2008openstreetmap}. The transmitter is positioned at the center of the scene at a height of 8.5\,m, mimicking a mmWave deployment.

\subsubsection*{Spatial Sampling Strategy}

Within this environment, \gls{ue} locations are sampled uniformly over a circular region of radius 100\,m centered at the transmitter. We retain only outdoor locations by performing geometric consistency checks against the building meshes to ensure that no sampled point lies inside a building structure. The resulting samples include both \gls{los} and \gls{nlos} conditions.

\subsubsection*{Channel Simulation}

For the selected outdoor points, the \gls{csi} is generated using Sionna RT v1.2~\cite{hoydis2023sionna}. The simulations are conducted at carrier frequencies of 3.5 and 28\,GHz. The network and ray-tracing configurations employed for generating the channel links between the \gls{bs} and the selected \glspl{ue} are summarized in Table~\ref{tab:network_rt_parameters}. For the 3.5\,GHz carrier frequency, the \gls{bs} latitude and longitude are shifted by 5\,m to place the transmitter on top of a building at 25\,m.

The OFDM channel in Sionna RT is constructed from the ray-traced propagation paths between the \gls{bs} and each \gls{ue}. For user $u$, the baseband-equivalent channel impulse response is written as
\begin{equation}
h_u(t)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,\delta\!\left(t-\tau_{u,\ell}\right),
\label{eq:cir_user}
\end{equation}
where $L_u$ is the number of valid propagation paths, $a_{u,\ell}\in\mathbb{C}$ is the complex coefficient of path $\ell$, and $\tau_{u,\ell}$ is the corresponding propagation delay.

The corresponding frequency-domain channel response is obtained as
\begin{equation}
H_u(f)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,e^{-j2\pi f \tau_{u,\ell}},
\label{eq:cfr_user}
\end{equation}
where $f$ denotes the frequency variable.

For an OFDM system with $K$ subcarriers, the channel coefficient on subcarrier $k$ is obtained by sampling \eqref{eq:cfr_user} at the subcarrier frequency $f_k$, i.e.,
\begin{equation}
H_u[k]=H_u(f_k)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,e^{-j2\pi f_k \tau_{u,\ell}},
\qquad k=0,\ldots,K-1,
\label{eq:ofdm_channel_user}
\end{equation}
where $f_k$ is the frequency of the $k$-th subcarrier. Therefore, the OFDM channel of each \gls{ue} is directly obtained from the ray-traced path gains and delays computed by Sionna RT.

\begin{comment}

\subsection{Dataset Generation}

%In this work, ground truth channel realizations are obtained via site-specific ray tracing based on a three-dimensional representation of the environment, including building geometries and material properties. For each \gls{ue} location, the Sionna ray tracer computes a set of propagation paths characterized by their delays, angles of departure and arrival, and complex coefficients, accounting for LoS, specular reflections, and diffraction mechanisms. Further details on the ray tracing configuration and simulation parameters are provided in} \colorbox{yellow}{Section~\ref{subsec:dataset_generation}

%The dataset is generated from a single dense urban scene extracted from a real cellular deployment. The selected environment spans an area of $250 \times 250$ meters and contains detailed three-dimensional building geometries obtained from \gls{osm}~\cite{haklay2008openstreetmap}. The transmitter is positioned at the center of the scene at a height of 8.5 meters, mimicking a mmWave deployment. 

%A two-dimensional representation of the considered environment is illustrated in Fig.~\ref{fig:single_scene_height_map}. 
%Each pixel encodes the height of the corresponding building footprint, yielding a structured image of the urban layout. This representation provides an explicit spatial description of the environment and can be used for visualization or auxiliary conditioning.

\paragraph{Spatial Sampling Strategy}
Within this environment, UE locations are sampled uniformly over a circular region of radius 100\,m centered at the transmitter. We retain only outdoor locations by performing geometric consistency checks against the building meshes to ensure that no sampled point lies inside a building structure. As a result, we have $\approx$ 40.000 samples including \gls{los} and \gls{nlos}. We note that both the source code and the dataset are publicly available\footnote{INSERT_GITHB_URL}.

%Among the outdoor points, we further select those exhibiting at least one line-of-sight (LoS) propagation path with respect to the transmitter. This constraint guarantees physically meaningful channel realizations and avoids degenerate cases dominated purely by deep non-line-of-sight attenuation. After applying the outdoor and LoS filtering criteria, the resulting dataset consists of approximately $13000$ valid UE locations.




\paragraph{Channel Simulation}
For the selected outdoor points, the \gls{csi} is generated using Sionna RT v1.2\cite{hoydis2023sionna}. The simulations are conducted at a carrier frequency of 3.5 and 28\,GHz. The network and RT configurations employed for generating the channel links between the BS and the selected UEs are summarized in Table \ref{tab:network_rt_parameters}. To make the simulations more realistic, we change the BS latitude and longitude location by 5 meters to place it on top of a building at 25 meters for the 3.5 GHz carrier frequency.

The OFDM channel in Sionna RT is constructed from the ray-traced propagation paths between the BS and each UE. For user $u$, the baseband-equivalent channel impulse response is written as
\begin{equation}
h_u(t)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,\delta\!\left(t-\tau_{u,\ell}\right),
\label{eq:cir_user}
\end{equation}
where $L_u$ is the number of valid propagation paths, $a_{u,\ell}\in\mathbb{C}$ is the complex coefficient of path $\ell$, and $\tau_{u,\ell}$ is the corresponding propagation delay.

The corresponding frequency-domain channel response is obtained as
\begin{equation}
H_u(f)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,e^{-j2\pi f \tau_{u,\ell}},
\label{eq:cfr_user}
\end{equation}
where $f$ denotes the frequency variable.

For an OFDM system with $K$ subcarriers, the channel coefficient on subcarrier $k$ is obtained by sampling \eqref{eq:cfr_user} at the subcarrier frequency $f_k$, i.e.,
\begin{equation}
H_u[k]=H_u(f_k)=\sum_{\ell=1}^{L_u} a_{u,\ell}\,e^{-j2\pi f_k \tau_{u,\ell}}, \qquad k=0,\ldots,K-1,
\label{eq:ofdm_channel_user}
\end{equation}
where $f_k$ is the frequency of the $k$-th subcarrier. Therefore, the OFDM channel of each UE is directly obtained from the ray-traced path gains and delays computed by Sionna RT.


\begin{table}[t]
\centering
\caption{Network and RT configuration parameters.}
\label{tab:network_rt_parameters}
\normalsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|p{0.30\columnwidth}|p{0.31\columnwidth}|p{0.31\columnwidth}|}
\hline
\textbf{Parameter} & \textbf{3.5 GHz} & \textbf{28 GHz} \\ 
% \hline
% Min/Max latitude & 51.5080, 51.5200 & 51.5080, 51.5200 \\ 
% \hline
% Min/Max longitude & -0.1450, -0.1250 & -0.1450, -0.1250 \\ 
\hline
Number of BSs & 1 & 1 \\ 
\hline
Number of UEs & $13 \times 10^{3}$ & $13 \times 10^{3}$ \\ 
\hline
Maximum UE--BS distance & 100\,m & 100\,m \\ 
\hline
BS antenna elements (row, column) & $1 \times 32$ & $1 \times 32$ \\ 
\hline
UE antenna elements (row, column) & $1 \times 4$ & $1 \times 4$ \\ 
\hline
Polarization & Vertical & Vertical \\ 
\hline
BS antenna pattern & Isotropic & Isotropic \\ 
\hline
UE antenna pattern & Isotropic & Isotropic \\ 
\hline
BS height & 8.5\,m & 8.5\,m \\ 
% \hline
% Carrier frequency & 28\,GHz & 28\,GHz \\ 
\hline
Number of shooting rays & $5 \times 10^{6}$ & $5 \times 10^{6}$ \\ 
\hline
Maximum ray bounces & 3 & 3 \\ 
\hline
Enabled propagation mechanisms & LoS, Specular reflection, diffraction & LoS, Specular reflection, diffraction \\ 
\hline
UE height & 1.5\,m & 1.5\,m \\ 
\hline
\end{tabular}
\end{table}

\end{comment}


\begin{comment}
The final dataset therefore consists of approximately 11\,000 samples, where each sample contains:
\begin{itemize}
    \item the beamspace channel tensor $H$,
    \item the corresponding UE coordinates $c_{\mathrm{xy}}=(x,y)$ within the 100\,m radius region,
    \item guarantees of outdoor placement and the presence of at least one LoS path.
\end{itemize}

\end{comment}






% \begin{itemize}
%   \item Describe the single-scene simulation pipeline and what varies across UE points (multipath randomness, blockers, etc.).
%   \item Dataset scale: $\sim$11k UE locations at 28~GHz (and optional repeat at 3.5~GHz).
%   \item Splits: emphasize \textbf{unseen UE locations} for test; keep conditioning identical across models.
% \end{itemize}
% \color{blue}
% \begin{itemize}
%     \item Sina update this
% \end{itemize}
% \color{black}

\subsection{Angular Spread Experiments}

To characterize the propagation properties of the considered reference channel datasets, we analyze the temporal and spatial dispersion of their multipath components through the RMS delay spread (DS) and the angular spreads, namely the azimuth spread of arrival and departure (ASA/ASD) and the zenith spread of arrival and departure (ZSA/ZSD). These metrics are computed from the path-level delays, angles, and complex coefficients of each BS--UE channel realization.

The RMS delay spread is obtained as
\begin{equation}
\bar{\tau}=\frac{\sum_n P_n \tau_n}{\sum_n P_n},
\qquad
\sigma_\tau=\sqrt{\frac{\sum_n P_n \tau_n^2}{\sum_n P_n}-\bar{\tau}^2},
\end{equation}
where $P_n=|a_n|^2$ is the power of the $n$-th path and $\tau_n$ its delay. The angular spreads are computed using the power-weighted circular formulation
\begin{equation}
\sigma_{\phi}=
\sqrt{-2\ln\left|
\frac{\sum_n P_n e^{j\phi_n}}{\sum_n P_n}
\right|},
\end{equation}
applied to AoA, AoD, ZoA, and ZoD to obtain ASA, ASD, ZSA, and ZSD, respectively.

Fig.~\ref{fig:cdf_spreads} shows the empirical CDFs of these five spread metrics for the considered 3GPP and Sionna RT datasets at 3.5~GHz and 28~GHz. The results indicate clear differences in the temporal and spatial structure of the channels. In particular, the 3GPP dataset at 3.5~GHz exhibits the largest delay spread, whereas the 28~GHz and RT cases are more concentrated at lower DS values. For the angular metrics, ASA is relatively similar across datasets, while ASD shows more pronounced differences, with the RT datasets exhibiting broader departure-angle dispersion. Moreover, ZSA and ZSD remain smaller than the azimuth spreads in all cases, confirming that most of the multipath energy is distributed mainly in the horizontal plane.

Overall, this analysis provides a compact description of the propagation structure of the reference datasets and highlights the differences between stochastic and site-specific channel modeling in both the delay and angular domains.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/Fig01_CDF_All_Spread_Metrics.png}
    \caption{\hl{Replace as discussed with Angel. 3 figures, one per data bucket, just AoD.} Empirical CDF of the considered spread metrics for the reference channel datasets. From left to right, the panels show the RMS delay spread (DS), azimuth spread of arrival (ASA), azimuth spread of departure (ASD), zenith spread of arrival (ZSA), and zenith spread of departure (ZSD) for the 3GPP and Sionna RT datasets at 3.5~GHz and 28~GHz.}
    \label{fig:cdf_spreads}
\end{figure*}


\subsection{Channel Rank}

Fig.~\ref{fig:effective_rank_bar} \red{reports the median effective rank} for the
ground-truth reference channels and the synthetic channels generated by cDDIM and cFMM under three evaluation conditions. 

In the LoS-only scenarios, all effective
rank values remain close to unity, which is consistent with the expected
single-dominant-mode behavior of LoS propagation. In the LoS-only scenarios, both cDDIM and cFMM closely follow the GT reference, with median effective-rank values remaining close to unity across both carrier frequencies. This confirms that the generated channels preserve the low-rank spatial structure of the reference LoS channels, although with a slight upward bias in the estimated spatial richness.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/Effective_Rank/combined_effective_rank_bar.png}
    \caption{Median effective rank comparison between the reference ground-truth channels and the synthetic channels generated by cDDIM and cFMM for different carrier frequencies and propagation conditions.}
    \label{fig:effective_rank_bar}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{Figures/Effective_Rank/combined_ks_distance_bar.png}
    \caption{KS distance between the effective-rank distributions of the GT channels and the generated ones for different carrier frequencies and propagation conditions.}
    \label{fig:ks_distance_effective_rank}
\end{figure}

\red{The slight increase observed for the generated channels suggests that cDDIM and
cFMM distribute a small fraction of the channel energy across secondary spatial
modes. This behavior is reasonable for generative models trained in a
normalized beamspace representation, where small reconstruction or sampling
errors may appear as weak diffuse components over non-dominant beams.
Nevertheless, the generated LoS channels remain in the same low-rank regime as
the ground-truth reference, indicating that the dominant spatial organization is
well preserved.}

\blue{It is important to emphasize that both cDDIM and cFMM are trained using only
$200$ GT ray tracing channel realizations. Despite this limited
training set, the generated LoS channels remain in the same low-rank regime as
the ground-truth reference, showing that the dominant spatial structure is
effectively captured. The slight increase in effective rank is therefore
expected, as generative models trained from few normalized beamspace samples
may introduce small variations over secondary spatial modes while still
preserving the main channel structure.}

In the mixed LoS+NLoS condition at $3.5$~GHz, the effective-rank values increase for all datasets, reflecting the richer spatial structure introduced by NLoS propagation. The generated channels follow the same trend, although they exhibit slightly higher median effective ranks than the GT reference. This behavior can be attributed to the heterogeneous nature of the pooled LoS+NLoS dataset: since the model learns from channel realizations with different spatial-rank characteristics, the generated samples may distribute energy more smoothly across secondary spatial modes. This effect is less visible in the LoS-only cases, where the propagation condition is more homogeneous.

Overall, the effective-rank results preserve the expected ordering of spatial richness across propagation conditions, with the mixed LoS+NLoS case exhibiting the highest values. At the same time, all values remain far from the full-rank regime, confirming that the generated channels maintain a physically plausible low-rank MIMO structure.

\begin{figure}[!t]
    \centering

    \includegraphics[width=\columnwidth]{Figures/Effective_Rank/effective_rank_cdf_28_GHz_LoS.png}
    \vspace{1mm}
    
    {\footnotesize (a) $28$~GHz LoS}
    
    \vspace{2mm}

    \includegraphics[width=\columnwidth]{Figures/Effective_Rank/effective_rank_cdf_3p5_GHz_LoS.png}
    \vspace{1mm}
    
    {\footnotesize (b) $3.5$~GHz LoS}
    
    \vspace{2mm}

    \includegraphics[width=\columnwidth]{Figures/Effective_Rank/effective_rank_cdf_3p5_GHz_LoSplusNLoS.png}
    \vspace{1mm}
    
    {\footnotesize (c) $3.5$~GHz LoS+NLoS}

    \caption{CDFs of the effective-rank distributions for the ground-truth Sionna~RT channels and the generated cDDIM and cFMM channels under different carrier frequencies and propagation conditions.}
    \label{fig:effective_rank_cdf_all}
\end{figure}
